Pure state tomography with parallel unentangled measurements

Quantum state tomography (QST) aims at estimating a quantum state from averaged quantum measurements made on copies of the state. Most quantum algorithms rely on QST at some point and it is a well explored topic in the literature, mostly for mixed states. In this paper we focus on the QST of a pure quantum state using parallel unentangled measurements. Pure states are a small but useful subset of all quantum states, their tomography requires fewer measurements and is essentially a phase recovery problem. Parallel unentangled measurements are easy to implement in practice because they allow the user to measure each qubit individually. We propose two sets of quantum measurements that one can make on a pure state as well as the algorithms that use the measurements outcomes in order to identify the state. We also discuss how those estimates can be fined tuned by finding the state that maximizes the likelihood of the measurements with different variants of the likelihood. The performances of the proposed three types of QST methods are validated by means of detailed numerical tests.

==> alphabet.tex <==
% Document LaTeX	Auteur : Guy Le Besnerais	Date : 25/05/94
% Modification : J.-F. Gio	(15/09/95)
%			        J.I. (format Latex 2e, taille adaptative 22/03/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab = vecteurs
% v pour bold droit : \Av = Matrice
% D pour droit : \AD
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace et amsmath)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}

%%%% NEW - NEW - %%%%% Small caps gras %%%% 05-06-98 %%%% JFG %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Merci \`a Caro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareFontShape{T1}{cmr}{bx}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}
% SC en bold (Hack !)
\DeclareFontShape{T1}{cmr}{b}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}%

\def\scb#1{\bfseries {\scshape #1}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% DEFINITIONS PRELIMINAIRES 

% definition pour \xspace
\def\XS{\xspace}

% Style gras italique (Necessite amsmath)
\def\sbm#1{\ensuremath{\boldsymbol{#1}}}               

% Style droit en math
\def\sdm#1{\ensuremath{\mathrm{#1}}}

% Style gras droit
\def\sbv#1{\ensuremath{\mathbf{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ALPHABET GRAS ITALIQUE
% Taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% ALPHABET GRAS ITALIQUE SOULIGNE
\def\Abu{\underline{\Ab}}  \def\abu{\underline{\ab}}
\def\Bbu{\underline{\Bb}}  \def\bbu{\underline{\bb}}
\def\Cbu{\underline{\Cb}}  \def\cbu{\underline{\cb}}
\def\Dbu{\underline{\Db}}  \def\dbu{\underline{\db}}
\def\Ebu{\underline{\Eb}}  \def\ebu{\underline{\eb}}
\def\Fbu{\underline{\Fb}}  \def\fbu{\underline{\fb}}
\def\Gbu{\underline{\Gb}}  \def\gbu{\underline{\gb}}
\def\Hbu{\underline{\Hb}}  \def\hbu{\underline{\hb}}
\def\Ibu{\underline{\Ib}}  \def\ibu{\underline{\ib}}
\def\Jbu{\underline{\Jb}}  \def\jbu{\underline{\jb}}
\def\Kbu{\underline{\Kb}}  \def\kbu{\underline{\kb}}
\def\Lbu{\underline{\Lb}}  \def\lbu{\underline{\lb}}
\def\Mbu{\underline{\Mb}}  \def\mbu{\underline{\mb}}
\def\Nbu{\underline{\Nb}}  \def\nbu{\underline{\nb}}
\def\Obu{\underline{\Ob}}  \def\obu{\underline{\ob}}
\def\Pbu{\underline{\Pb}}  \def\pbu{\underline{\pb}}
\def\Qbu{\underline{\Qb}}  \def\qbu{\underline{\qb}}
\def\Rbu{\underline{\Rb}}  \def\rbu{\underline{\rb}}
\def\Sbu{\underline{\Sb}}  \def\sbu{\underline{\sb}}
\def\Tbu{\underline{\Tb}}  \def\tbu{\underline{\tb}}
\def\Ubu{\underline{\Ub}}  \def\ubu{\underline{\ub}}
\def\Vbu{\underline{\Vb}}  \def\vbu{\underline{\vb}}
\def\Wbu{\underline{\Wb}}  \def\wbu{\underline{\wb}}
\def\Xbu{\underline{\Xb}}  \def\xbu{\underline{\xb}}
\def\Ybu{\underline{\Yb}}  \def\ybu{\underline{\yb}}
\def\Zbu{\underline{\Zb}}  \def\zbu{\underline{\zb}}

% ALPHABET CURSIF
% Cursif(majuscules), taille adaptative

\def\Ac{{\ensuremath{\mathcal{A}}}\XS}
\def\Bc{{\ensuremath{\mathcal{B}}}\XS}
\def\Cc{{\ensuremath{\mathcal{C}}}\XS}
\def\Dc{{\ensuremath{\mathcal{D}}}\XS}
\def\Ec{{\ensuremath{\mathcal{E}}}\XS}
\def\Fc{{\ensuremath{\mathcal{F}}}\XS}
\def\Gc{{\ensuremath{\mathcal{G}}}\XS}
\def\Hc{{\ensuremath{\mathcal{H}}}\XS}
\def\Ic{{\ensuremath{\mathcal{I}}}\XS}
\def\Jc{{\ensuremath{\mathcal{J}}}\XS}
\def\Kc{{\ensuremath{\mathcal{K}}}\XS}
\def\Lc{{\ensuremath{\mathcal{L}}}\XS}
\def\Mc{{\ensuremath{\mathcal{M}}}\XS}
\def\Nc{{\ensuremath{\mathcal{N}}}\XS}
\def\Oc{{\ensuremath{\mathcal{O}}}\XS}
\def\Pc{{\ensuremath{\mathcal{P}}}\XS}
\def\Qc{{\ensuremath{\mathcal{Q}}}\XS}
\def\Rc{{\ensuremath{\mathcal{R}}}\XS}
\def\Sc{{\ensuremath{\mathcal{S}}}\XS}
\def\Tc{{\ensuremath{\mathcal{T}}}\XS}
\def\Uc{{\ensuremath{\mathcal{U}}}\XS}
\def\Vc{{\ensuremath{\mathcal{V}}}\XS}
\def\Wc{{\ensuremath{\mathcal{W}}}\XS}
\def\Xc{{\ensuremath{\mathcal{X}}}\XS}
\def\Yc{{\ensuremath{\mathcal{Y}}}\XS}
\def\Zc{{\ensuremath{\mathcal{Z}}}\XS}

% Lettres cursives grasses (majuscules)
%
\def\Acb{{\sbm{\mathcal{A}}}\XS}
\def\Bcb{{\sbm{\mathcal{B}}}\XS}
\def\Ccb{{\sbm{\mathcal{C}}}\XS}
\def\Dcb{{\sbm{\mathcal{D}}}\XS}
\def\Ecb{{\sbm{\mathcal{E}}}\XS}
\def\Fcb{{\sbm{\mathcal{F}}}\XS}
\def\Gcb{{\sbm{\mathcal{G}}}\XS}
\def\Hcb{{\sbm{\mathcal{H}}}\XS}
\def\Icb{{\sbm{\mathcal{I}}}\XS}
\def\Jcb{{\sbm{\mathcal{J}}}\XS}
\def\Kcb{{\sbm{\mathcal{K}}}\XS}
\def\Lcb{{\sbm{\mathcal{L}}}\XS}
\def\Mcb{{\sbm{\mathcal{M}}}\XS}
\def\Ncb{{\sbm{\mathcal{N}}}\XS}
\def\Ocb{{\sbm{\mathcal{O}}}\XS}
\def\Pcb{{\sbm{\mathcal{P}}}\XS}
\def\Qcb{{\sbm{\mathcal{Q}}}\XS}
\def\Rcb{{\sbm{\mathcal{R}}}\XS}
\def\Scb{{\sbm{\mathcal{S}}}\XS}
\def\Tcb{{\sbm{\mathcal{T}}}\XS}
\def\Ucb{{\sbm{\mathcal{U}}}\XS}
\def\Vcb{{\sbm{\mathcal{V}}}\XS}
\def\Wcb{{\sbm{\mathcal{W}}}\XS}
\def\Xcb{{\sbm{\mathcal{X}}}\XS}
\def\Ycb{{\sbm{\mathcal{Y}}}\XS}
\def\Zcb{{\sbm{\mathcal{Z}}}\XS}


% ALPHABET DROIT EN MATHS
% Taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT
% Permet d'obtenir des caracteres droits directement 
% en mode math ou pas math.
% (Un peu moins utile peut \^eetre)

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% ALPHABET GREC GRAS 
% Enrichie, completee et modifi\'ee par J.-F. Gio.
% Taille adaptative !

\def\alphab      {{\sbm{\alpha}}\XS}
\def\betab       {{\sbm{\beta}}\XS}
\def\gammab      {{\sbm{\gamma}}\XS}	  \def\Gammab    {{\sbm{\Gamma}}\XS}
\def\deltab      {{\sbm{\delta}}\XS}	  \def\Deltab    {{\sbm{\Delta}}\XS}
\def\epsilonb    {{\sbm{\epsilon}}\XS}
\def\varepsilonb {{\sbm{\varepsilon}}\XS}
\def\etab        {{\sbm{\eta}}\XS}
\def\thetab      {{\sbm{\theta}}\XS}	  \def\Thetab    {{\sbm{\Theta}}\XS}
\def\varthetab   {{\sbm{\vartheta}}\XS}
\def\iotab       {{\sbm{\iota}}\XS}
\def\kappab      {{\sbm{\kappa}}\XS}
\def\lambdab     {{\sbm{\lambda}}\XS}    \def\Lambdab   {{\sbm{\Lambda}}\XS}
\def\mub         {{\sbm{\mu}}\XS}
\def\nub         {{\sbm{\nu}}\XS}
\def\xib         {{\sbm{\xi}}\XS}		  \def\Xib  	  {{\sbm{\Xi}}\XS}
\def\pib         {{\sbm{\pi}}\XS}		  \def\Pib  	  {{\sbm{\Pi}}\XS}
\def\varpib      {{\sbm{\varpi}}\XS}
\def\rhob        {{\sbm{\rho}}\XS}
\def\varrhob     {{\sbm{\varrho}}\XS}
\def\sigmab      {{\sbm{\sigma}}\XS}	  \def\Sigmab    {{\sbm{\Sigma}}\XS}
\def\varsigmab   {{\sbm{\varsigma}}\XS}  \def\Varsigmab {{\sbm{\Varsigma}}\XS}
\def\phib        {{\sbm{\phi}}\XS}  	  \def\Phib 	  {{\sbm{\Phi}}\XS}
\def\varphib     {{\sbm{\varphi}}\XS}
\def\chib        {{\sbm{\chi}}\XS}
\def\psib        {{\sbm{\psi}}\XS}  	  \def\Psib 	  {{\sbm{\Psi}}\XS}
\def\omegab      {{\sbm{\omega}}\XS}	  \def\Omegab    {{\sbm{\Omega}}\XS}
\def\taub        {{\sbm{\tau}}\XS}
\def\upsilonb    {{\sbm{\upsilon}}\XS}   \def\Upsilonb  {{\sbm{\Upsilon}}\XS}
\def\zetab       {{\sbm{\zeta}}\XS}

% ALPHABET GREC GRAS SOULIGNE
% Enrichie, completee et modifi\'ee par J.-F. Gio.
% Taille adaptative !

\def\alphabu{\underline{\alphab}}
\def\betabu{\underline{\betab}}
\def\gammabu{\underline{\gammab}}
\def\deltabu{\underline{\deltab}}
\def\epsilonbu{\underline{\epsilonb}}
\def\varepsilonbu{\underline{\varepsilonb}}
\def\etabu{\underline{\etab}}
\def\thetabu{\underline{\thetab}}
\def\varthetabu {\underline{\varthetab}}
\def\iotabu{\underline{\iotab}}
\def\kappabu{\underline{\kappab}}
\def\lambdabu{\underline{\lambdab}}
\def\mubu{\underline{\mub}}
\def\nubu{\underline{\nub}}
\def\xibu{\underline{\xib}}
\def\pibu{\underline{\pib}}
\def\varpibu{\underline{\varpib}}
\def\rhobu{\underline{\rhob}}
\def\varrhobu{\underline{\varrho}}
\def\sigmabu{\underline{\sigmab}}
\def\varsigmabu{\underline{\varsigmab}}
\def\phibu{\underline{\phib}}
\def\varphibu{\underline{\varphib}}
\def\chibu{\underline{\chib}}
\def\psibu{\underline{\psib}}
\def\omegabu{\underline{\omegab}}
\def\taubu{\underline{\taub}}
\def\upsilonbu{\underline{\upsilonb}}
\def\zetabu{\underline{\zetab}}



% CHIFFRES
% Gras, taille adaptative

\def\zerob	 {{\sbv{0}}\XS} \def\zerobu{\underline{\zerob}}
\def\unb		 {{\sbv{1}}\XS}
\def\deuxb	 {{\sbv{2}}\XS}
\def\troisb	 {{\sbv{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}
\def\cinqb	 {{\sbv{5}}\XS}
\def\sixb	 {{\sbv{6}}\XS}
\def\septb	 {{\sbv{7}}\XS}
\def\huitb	 {{\sbv{8}}\XS}
\def\neufb	 {{\sbv{9}}\XS}


% QUELQUES ENSEMBLES
% Taille adaptative

\def\eC{{\ensuremath{\mathbb C}}\XS}
\def\eE{{\ensuremath{\mathbb E}}\XS}
\def\eN{{\ensuremath{\mathbb N}}\XS}
\def\eR{{\ensuremath{\mathbb R}}\XS}
\def\eZ{{\ensuremath{\mathbb Z}}\XS}
\def\eC{{\ensuremath{\mathbb C}}\XS}
\def\eQ{{\ensuremath{\mathbb Q}}\XS}

